Testing for Global Network Structure Using Small Subgraph Statistics

We study the problem of testing for community structure in networks using relations between the observed frequencies of small subgraphs. We propose a simple test for the existence of communities based only on the frequencies of three-node subgraphs. The test statistic is shown to be asymptotically normal under a null assumption of no community structure, and to have power approaching one under a composite alternative hypothesis of a degree-corrected stochastic block model. We also derive a version of the test that applies to multivariate Gaussian data. Our approach achieves near-optimal detection rates for the presence of community structure, in regimes where the signal-to-noise is too weak to explicitly estimate the communities themselves, using existing computationally efficient algorithms. We demonstrate how the method can be effective for detecting structure in social networks, citation networks for scientific articles, and correlations of stock returns between companies on the S\&P 500.

==> fb100-sample.tex <==

\begin{figure}[!ht]
\begin{center}
\begin{tabular}{cccc}
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-small-p-1} &
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-small-p-2} &
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-small-p-3} &
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-small-p-4} \\
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-small-p-5} &
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-small-p-6} &
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-small-p-7} &
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-small-p-8} \\
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-small-p-9} &
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-small-p-10} &
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-small-p-11} &
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-small-p-12} \\
\end{tabular}
\vskip20pt
\centerline{\hbox to 5in{\hrulefill}}
\vskip20pt
\begin{tabular}{cccc}
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-large-p-5} &
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-large-p-6} &
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-large-p-7} &
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-large-p-8} \\
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-large-p-9} &
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-large-p-10} &
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-large-p-11} &
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-large-p-12} \\
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-large-p-13} &
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-large-p-14} &
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-large-p-15} &
\includegraphics[width=.17\textwidth]{fb100/Carnegie49-large-p-16} \\
\end{tabular}
\caption{Facebook neighborhood graphs, each with between 30 and 40 nodes,
  extracted from the Carnegie Mellon University portion of the
  Facebook 100 dataset. Top: 12 randomly selected graphs with  p-values smaller than
  $10^{-12}$, under the EZ test. Bottom: 12 graphs
  with p-values larger than 0.2. The results for other
  universities are similar. Community structure is readily apparent in
  the top graphs, and lacking in the bottom graphs.}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=.45\textwidth]{fb100/Carnegie49-pvalue-histogram}&
\includegraphics[width=.45\textwidth]{fb100/Carnegie49-pvalue-histogram}
\end{tabular}
\end{center}
\caption{Histograms of p-values of the Facebook graphs...}
\end{figure}


==> relations.tex <==
%!TEX root = testing-networks.tex

\section{Relations Between Small Subgraph Frequencies}\label{sec:equations}


We now describe the basic relations between small subgraph
probabilities that we study.  There are four three-node subgraphs to consider: The empty graph (\shape{\emptyshape}), a
single edge (\shape{\edgeshape}), the V-shape
\hbox{(\shape{\Vshape})}, and the triangle (\shape{\triangleshape}).
Let $ A = (A_{ij})_{1\leq i<j\leq n}$ denote the adjacency matrix 
for a given undirected network on $n$ nodes.
We shall use subscripts that indicate the number of edges in the 
subgraph.  Thus, the relative frequency of triangles among 
all three-node subgraphs is 
$$\hat{F}_3=\frac{1}{{n\choose 3}}\sum_{1\leq i<j<k\leq
  n}A_{ij}A_{jk}A_{ki},$$
the $V$-shape frequency is 
$$\hat{F}_2=\frac{1}{{n\choose 3}}\sum_{1\leq i<j<k\leq n}\bigl\{(1-A_{ij})A_{jk}A_{ki}+A_{ij}(1-A_{jk})A_{ki}+A_{ij}A_{jk}(1-A_{ki})\bigr\},$$
the single edge frequency is 
$$\hat{F}_1=\frac{1}{{n\choose 3}}\sum_{1\leq i<j<k\leq n}\bigl\{(1-A_{ij})(1-A_{jk})A_{ki}+A_{ij}(1-A_{jk})(1-A_{ki})+(1-A_{ij})A_{jk}(1-A_{ki})\bigr\},$$
and the empty graph frequency is 
$$\hat{F}_0=\frac{1}{{n\choose 3}}\sum_{1\leq i<j<k\leq
  n}(1-A_{ij})(1-A_{jk})(1-A_{ki}).$$
Under an Erd\H{o}s-R\'{e}nyi model with edge probability $p$, the
population subgraph frequencies of the above four shapes are easily
seen to be
\begin{equation}
\mathbb{E}\hat{F}_3=p^3,\quad \mathbb{E}\hat{F}_2=3p^2(1-p),\quad\mathbb{E}\hat{F}_1=3p(1-p)^2,\quad\text{and}\quad \mathbb{E}\hat{F}_0=(1-p)^3.\label{eq:pop-freq}
\end{equation}
These expressions suggest that the subgraph frequencies can also be
estimated plugging in the empirical edge frequency
\begin{equation}
\hat{p}=\frac{1}{{n\choose 2}}\sum_{1\leq i<j\leq n}A_{ij}.\label{eq:p-hat}
\end{equation}
Under the Erd\H{o}s-R\'{e}nyi model, one can expect that the two ways
of estimating subgraph frequencies are close. This leads us to study the following four relations:
\begin{eqnarray*}
T_0 &=& (1-\hat{p})^3-\hat{F}_0,\\
T_1 &=& 3\hat{p}(1-\hat{p})^2-\hat{F}_1, \\
T_2 &=& 3\hat{p}^2(1-\hat{p})-\hat{F}_2, \\
T_3 &=& \hat{p}^3-\hat{F}_3.
\end{eqnarray*}
The quantities $T_0$, $T_1$, $T_2$ and $T_3$ are the differences
between the empirical subgraph frequencies and their plugin estimates.
It is easy to see that $T_0+T_1+T_2+T_3=0$; thus, there are at most
three degrees of freedom among the four equations. The following
proposition shows that for a sparse Erd\H{o}s-R\'{e}nyi graph, the
asymptotic number of degrees of freedom is actually only two.

\begin{proposition}\label{prop:corr}
Suppose that $p=o(1)$. Then
$$\Corr(T_2,T_3)=o(1),\quad \Corr(T_1,T_3)=o(1),\quad\text{and}\quad \Corr(T_1,T_2)=1+o(1),$$
where $o(1)$ indicates a quantity that converges to $0$ as $n\rightarrow\infty$.
\end{proposition}

The proposition shows that in order to understand the asymptotic
distribution of $T_0$, $T_1$, $T_2$, and $T_3$, it is sufficient to
study the asymptotic distribution of $(T_2,T_3)$.  However, this is
not a trivial task. Take $T_3$ for example. Although the leading term in
the expansion of $\hat{p}^3$ can be easily shown to be asymptotically
Gaussian using the delta method, and the leading term in the
expansion of $\hat{F}_3$ can also be shown to be asymptotically
Gaussian using the theory of incomplete U-statistics
\citep{nowicki1988subgraph,janson1991asymptotic}, the two leading
terms exactly cancel each other in $T_3$.  
It is therefore somewhat surprising that the joint
asymptotic distribution of $(T_2,T_3)$ is still Gaussian, as shown
in the next theorem.

\begin{theorem}\label{thm:vanilla}
Assume $(1-p)^{-1}=O(1)$ and $np\rightarrow\infty$. Then we have
$$\sqrt{{n\choose 3}}\Sigma_p^{-1/2}\begin{pmatrix}
T_2\\
T_3
\end{pmatrix}\leadsto N\left(\begin{pmatrix}
0 \\
0
\end{pmatrix},\begin{pmatrix}
1 & 0 \\
0 & 1
\end{pmatrix}\right),$$
where
\begin{equation} \label{eq:cov-def}
\Sigma_p=\begin{pmatrix}
3p^2(1-p)^2(1-3p)^2+9p^3(1-p)^3 & -6p^4(1-p)^2 \\
-6p^4(1-p)^2 & p^3(1-p)^3+3p^4(1-p)^2
\end{pmatrix}.
\end{equation}
\end{theorem}

The theorem gives a precise characterization of the asymptotic distribution of $(T_2,T_3)$. The condition $np\rightarrow\infty$ means that the network has a diverging degree. By the covariance structure (\ref{eq:cov-def}), it is easy to check that when $p=o(1)$, we have
$$\Corr(T_2,T_3)=\frac{\Cov(T_2,T_3)}{\sqrt{\Var(T_2)}\sqrt{\Var(T_3)}}=O(p^{3/2})=o(1),$$
which is consistent with Proposition \ref{prop:corr}.
The fact that $T_2$ and $T_3$ are asymptotically independent under
this scaling of $p$ suggests that one can build a chi-squared test to test whether a given network is generated by an Erd\H{o}s-R\'{e}nyi model. The proper normalization factor in the chi-squared test can be estimated using the empirical edge frequency (\ref{eq:p-hat}).

\begin{corollary}\label{cor:chi}
Assume $p=o(1)$ and $np\rightarrow\infty$. Then 
\begin{equation}
T^2=:{n\choose
  3}\left(\frac{T_2^2}{3\hat{p}^2(1-\hat{p})^2(1-3\hat{p})^2+9\hat{p}^3(1-\hat{p})^3}
+ \frac{T_3^2}{\hat{p}^3(1-\hat{p})^3+3\hat{p}^4(1-\hat{p})^2}\right)\leadsto \chi_2^2.\label{eq:chi^2}
\end{equation}
\end{corollary}

The natural $\alpha$-level test statistic is defined as
\begin{equation}
\phi_{\alpha}=\mathbb{I}\{T^2>C_{\alpha}\},\label{eq:test-alpha}
\end{equation}
where $C_{\alpha}$ is a constant satisfying
$\mathbb{P}(\chi_2^2>C_{\alpha})=\alpha$. Corollary \ref{cor:chi} then
implies that the Type-I error $\mathbb{P}_0\phi_{\alpha}$ is
asymptotically at the level $\alpha$ under an Erd\H{o}s-R\'{e}nyi
model. 


